Visual Ground Truth Construction as Faceted Classification

Recent work in Machine Learning and Computer Vision has provided evidence of systematic design flaws in the development of major object recognition benchmark datasets. One such example is ImageNet, wherein, for several categories of images, there are incongruences between the objects they represent and the labels used to annotate them. The consequences of this problem are major, in particular considering the large number of machine learning applications, not least those based on Deep Neural Networks, that have been trained on these datasets. In this paper we posit the problem to be the lack of a knowledge representation (KR) methodology providing the foundations for the construction of these ground truth benchmark datasets. Accordingly, we propose a solution articulated in three main steps: (i) deconstructing the object recognition process in four ordered stages grounded in the philosophical theory of teleosemantics; (ii) based on such stratification, proposing a novel four-phased methodology for organizing objects in classification hierarchies according to their visual properties; and (iii) performing such classification according to the faceted classification paradigm. The key novelty of our approach lies in the fact that we construct the classification hierarchies from visual properties exploiting visual genus-differentiae, and not from linguistically grounded properties. The proposed approach is validated by a set of experiments on the ImageNet hierarchy of musical experiments.

==> S5.tex <==
% \textbf{P1:} Pseudocode \\
% \textbf{P2:} Description (1) \\
% \textbf{P3:} Description (2) \\
% \textbf{P4:} Mapping to Section (2)

% \begin{algorithm}[H]
% \caption{Top-level loop}
% \begin{algorithmic}[1] 
% \Procedure{build\_subsumption\_hierarchy}{ }
% \While{$True$}
%     \State $E \gets \Call{Perceive}{ }$ \label{alg1:lin:perceive}
%     \State $ \Call{vertical\_recursion}{memory, E}$ \label{alg1:lin:verticalrecursion}
% \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{Vertical recursion}
% \begin{algorithmic}[1] 
% \Procedure{vertical\_recursion}{$root, encounter$}
%     \State $same\_genus\_count \gets 0$ \label{alg2:initcounter}
%     \ForEach{$child \in root.children$} \label{alg2:foreach}
%         \If{\Call{Genus}{$child, encounter$}} \label{alg2:ifgenusholds}
%             \State \Call{horizontal\_recursion}{$root, child, encounter$} \label{alg2:horizontalrecursion}
%             \State $ same\_genus\_count \gets same\_genus\_count +1$ \label{alg2:updatecounter}
%         \EndIf
%     \EndFor
%     \If{$same\_genus\_count = 0$} \label{alg2:ifnogenus}
%         \State \Call{AddChild}{$root, encounter$} \label{alg2:createchild}
%     \EndIf
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Horizontal recursion}
% \begin{algorithmic}[1] 
% \Procedure{horizontal\_recursion}{$root, node, encounter$}
%     % \State $differentia \gets $\Call{DifferentiaObj}{$child, encounter$}
%     \If{\Not \Call{Differentia}{$node, encounter$}} \label{alg3:ifnotdifferentia}
%         \State \Call{UpdateNode}{$node, encounter$} \label{alg3:updateequal}
%     \Else
%         \State $genus \gets $\Call{GenusObj}{$node, encounter$} \label{alg3:getgenus}
%         \If{$node = genus$} \label{alg3:ifnodeequalsgenus}
%             % \State $common \gets$ \Call{Intersection}{$encounter, genus$} \label{alg3:interencountergenus}
%             \State \Call{UpdateNode}{$node, encounter$} \label{alg3:updatenodecommon}
%             % \State $encounter \gets$ \Call{Difference}{$encounter, common$} \label{alg3:diffencountercommon}
%             \State \Call{vertical\_recursion}{$node, encounter$} \label{alg3:verticalrecursion}
%         \ElsIf{$encounter = genus$} \label{alg3:ifencounterequalsgenus}
%             \State \Call{RemoveChild}{$root, node$} \label{alg3:removechildnode}
%             \State $new\_node \gets$\Call{AddChild}{$root, encounter$} \label{alg3:addchildencounter}
%             % \State $common \gets$ \Call{Intersection}{$node, genus$} \label{alg3:intersectionnodegenus}
%             \State \Call{UpdateNode}{$new\_node, node$} \label{alg3:updatenewnodecommon}
%             % \State $node \gets$\Call{Difference}{$node, common$} \label{alg3:differencenodecommon}
%             \State \Call{AddChild}{$new\_node, node$} \label{alg3:addchildnode}
%         \Else
%             \State \Call{RemoveChild}{$root, node$} \label{alg3:removechildnode2}
%             \State $genus\_node \gets$ \Call{AddChild}{$root, genus$} \label{alg3:addchildgenus}
%             % \State $common \gets$ \Call{Intersection}{$node, genus$} \label{alg3:intersectionnodegenus2}
%             % \State $node \gets$ \Call{Difference}{$node, common$} \label{alg3:differencenodecommon2}
%             % \State $common \gets$ \Call{Intersection}{$encounter, genus$} \label{alg3:intersectionencountergenus}
%             % \State $encounter \gets$ \Call{Difference}{$encounter, common$} \label{alg3:differenceencountercommon}
%             \State \Call{AddChild}{$genus\_node, node$} \label{alg3:addchildgenusnode}
%             \State \Call{AddChild}{$genus\_node, encounter$} \label{alg3:addchildgenusencounter}
%         \EndIf
%     \EndIf
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}
